Understanding GNN Computational Graph: A Coordinated Computation, IO, and Memory Perspective

Graph Neural Networks (GNNs) have been widely used in various domains, and GNNs with sophisticated computational graph lead to higher latency and larger memory consumption. Optimizing the GNN computational graph suffers from: (1) Redundant neural operator computation. The same data are propagated through the graph structure to perform the same neural operation multiple times in GNNs, leading to redundant computation which accounts for 92.4% of total operators. (2) Inconsistent thread mapping. Efficient thread mapping schemes for vertex-centric and edge-centric operators are different. This inconsistency prohibits operator fusion to reduce memory IO. (3) Excessive intermediate data. For GNN training which is usually performed concurrently with inference, intermediate data must be stored for the backward pass, consuming 91.9% of the total memory requirement. To tackle these challenges, we propose following designs to optimize the GNN computational graph from a novel coordinated computation, IO, and memory perspective: (1) Propagation-postponed operator reorganization. We reorganize operators to perform neural operations before the propagation, thus the redundant computation is eliminated. (2) Unified thread mapping for fusion. We propose a unified thread mapping scheme for both vertex- and edge-centric operators to enable fusion and reduce IO. (3) Intermediate data recomputation. Intermediate data are recomputed during the backward pass to reduce the total memory consumption. Extensive experimental results on three typical GNN models show that, we achieve up to 2.75x end-to-end speedup, 6.89x less memory IO, and 7.73x less memory consumption over state-of-the-art frameworks.

==> tex/implementation.tex <==
\section{Evaluation}
% In this section, we apply our methodology to three GNN models.

% \subsection{GATConv}


% The mathematical definition of one GATConv layer is shown in Eguation \ref{eq:gat1} and \ref{eq:gat2}. The computational graph of one GATConv layer is shown in figure.


% \begin{equation}\label{eq:gat1}
%     h_{i}^{(l+1)}=\sum_{j \in \mathcal{N}(i)} e_{ij} W^{(l)} h_{j}^{(l)}
% \end{equation}

% \begin{equation}\label{eq:gat2}
%     e_{i j}^{l} &=\operatorname{softmax}_{i}\left(\operatorname{LeakyReLU}\left(\vec{a}^{T}\left[W h_{i} \| W h_{j}\right]\right)\right)
% \end{equation}




% \subsubsection{Computational Graph DSE}
% We perform computational graph design space exploration and find that the computational graph is already a redundency-free MLP-GPA procedure, so no reorganization to the computational graph is needed.

% \textbf{MLP phase.} Several neural operators are first performed to compute the "attention" value. Assume the input node feature vectors are concatenated into a feature matrix $\boldsymbol{H}^{(l)} \in \mathbb{R}^{n \times f^{(l)}}$. We first perform a dense matrix matrix multiplication to transform this feature matrix into $\widetilde{\boldsymbol{H}^{(l)}}=\boldsymbol{H}^{(l)}\times \boldsymbol{W}^{(l)} \in \mathbb{R}^{n\times f^{(l+1)}}$ with torch.nn.linear. Follow the idea of DGL's implementation, we decompose the weight vector ${\boldsymbol{a}}\in \mathbb{R}^{2f^{(l+1)}}$ into $\left[\boldsymbol{a}_l||\boldsymbol{a}_r \right]$ and compute attention scores $\boldsymbol{A}_l=\widetilde{\boldsymbol{H}^{(l)}}\times\boldsymbol{a}_l\in \mathbb{R}^{n \times 1}$ and $\boldsymbol{A}_r=\widetilde{\boldsymbol{H}^{(l)}}\times\boldsymbol{a}_r\in \mathbb{R}^{n \times 1}$.

% \textbf{Message-generation phase}. Messages $\boldsymbol{M}_0\in\mathbb{R}^{n} $ are generated by $$\boldsymbol{M}_0=\operatorname{u\_add\_v}(\boldsymbol{A}_l,\boldsymbol{A}_r)$$

% \textbf{Message-passing phase}. An one-edge-to-one-edge operator is first applied to generate $$\boldsymbol{M_1}=\operatorname{LeakyReLU}(\boldsymbol{M}_0) \in\mathbb{R}^{n} $$ followed by a many-edge-to-many-edge operator to generate $$\boldsymbol{M_2}=\operatorname{edge\_softmax}(\boldsymbol{M}_1)\in\mathbb{R}^{n} $$as in Equation \ref{eq:gat2}.

% \textbf{Message-aggregation phase}. An edge-to-node operator, reduce\_sum, is performed to generate $$\boldsymbol{H}^{(l+1)}=\operatorname{reduce\_sum}(\boldsymbol{M_2},\widetilde{\boldsymbol{H}^{(l)}}) \in \mathbb{R}^{n \times f^{(l+1)}}$$ as in Equation \ref{eq:gat1}.



% \subsubsection{Fusion}
% We apply Lemma \ref{lemma:6} to fuse leakyrelu and edge\_softmax into one many-edge-to-many-edge operator. Then Lemma \ref{lemma:2} and \ref{lemma:3} are applied to fuse the GPA procedure into one operator.


% There are three intermediate variables needed for backward in the GPA procedure: $\boldsymbol{M_0}$, $\boldsymbol{M_1}$ and $\boldsymbol{M_2}$. As $\boldsymbol{M_0}$ and $\boldsymbol{M_1}$ can be computed within $O(1)$, the \textit{recompute} technique is applied. $\boldsymbol{M_3}$ takes $O(e/n)$ to compute, because we need to first compute the sum of the messages in the neighborhood as the denominator in softmax. By apply the \textit{cache and recompute} technique, we cache this sum as $\boldsymbol{M'_3}$ and the overhead of recompute is reduced to an affordable $O(1)$.

% \subsubsection{Implementation}


% \subsubsection{Evaluation}

% Before fusion, there are 3 neural operators and 4 GNN operators. The total memory space for saving the intermediate variable is $nf+n+n+e+e+e+nf=(2f+2)n+3e$.

% After fusion, there are still 3 neural operators but only 1 GNN operator, which is our fused operator. The total memory space for saving the intermediate variable is reduced to $nf+n+n+n+nf=(2f+3)n$.

% \subsection{EdgeConv}
% The mathematical definition of one EdgeConv layer is shown in Equation \ref{eq:edgeconv}.

% \begin{equation}\label{eq:edgeconv}
%     h_{i}^{(l+1)}=\max _{j \in \mathcal{N}(i)}\left(\Theta \cdot\left(h_{j}^{(l)}-h_{i}^{(l)}\right)+\Phi \cdot h_{i}^{(l)}\right)
% \end{equation}


% where $\mathcal{N}(i)$ is the neighbor of $i . \Theta$ and $\Phi$ are linear layers.

% \subsubsection{Computational Graph Analysis}
% In SOTA gnn framework DGL, one edgeconv layer is computed as shown in figure. There is no MLP phase in the edgeconv. Define the input node feature matrices as $ \boldsymbol{H}^{(l)}\in\mathbb{R}^{n\times f}$. The $(h_j^{(l)}-h_i^{(l)})$ in Equation \ref{eq:edgeconv} is computed by

% $$\boldsymbol{E}^{(l)}=\operatorname{u\_sub\_v}\left(\boldsymbol{H}^{(l)}\right)\in\mathbb{R}^{e\times f^{(l)}}$$

% followed by one MLP 
% $$\boldsymbol{E}_\Theta^{(l)}=\Theta \cdot \boldsymbol{E}^{(l)}\in\mathbb{R}^{e\times f^{(l+1)}}$$

% Another MLP is performed to compute $\Phi \cdot h_{i}^{(l)$ in Equation \ref{eq:edgeconv}

% $$\boldsymbol{N}_\Phi^{(l)}=\Phi \cdot \boldsymbol{H}^{(l)}\in\mathbb{R}^{n\times f^{(l+1)}}$$

% followed by

% $$\boldsymbol{E}_{\Theta+\Phi}^{(l)}=\operatorname{e\_add\_v}\left(\boldsymbol{E}_\Theta^{(l)},\boldsymbol{N}_\Phi^{(l)}\right)\in\mathbb{R}^{e\times f^{(l+1)}}$$

% In the end, a reduce function is called to update the node features

% $$\boldsymbol{H}^{(l+1)}=\operatorname{reduce\_max}\left(\boldsymbol{E}_{\Theta+\Phi}^{(l)}\right)\in\mathbb{R}^{n\times f^{(l+1)}}$$

% \subsubsection{Computational Graph DSE}
% In the original computational graph, MLP is performed to the edge data. We find Equation \ref{eq:edgeconv} can be written as
% \begin{equation}\label{eq:edgeconv_our}
%     h_{i}^{(l+1)}=\max _{j \in \mathcal{N}(i)}\left(\Theta \cdot h_{j}^{(l)}+\left(\Phi-\Theta\right) \cdot h_{i}^{(l)}\right)
% \end{equation}
% Therefore, we can reorganize the computational graph as MLP-GPA and only perform MLP to node data instead of edge data.

% \textbf{MLP phase:}
% $$\boldsymbol{H}_{\Phi-\Theta}^{(l)}=\left(\Phi-\Theta\right)\cdot\boldsymbol{H}^{(l)},\ \ 
% \boldsymbol{H}_{\Theta}^{(l)}=\Theta\cdot\boldsymbol{H}^{(l)}\in\mathbb{R}^{n\times f^{(l+1)}}
% $$

% \textbf{Message-generation:}
% $$\boldsymbol{M}=\operatorname{u\_add\_v}\left(\boldsymbol{H}_{\Phi-\Theta}^{(l)},\boldsymbol{H}_{\Theta}^{(l)}\right)\in\mathbb{R}^{e\times f^{(l+1)}}$$

% \textbf{Message-passing:} none.

% \textbf{Message-aggregation:}
% $$\boldsymbol{H}^{(l+1)}=\operatorname{reduce\_max}\left(\boldsymbol{M}\right)\in\mathbb{R}^{n\times f^{(l+1)}}$$

% \subsubsection{Forward Fusion}
% We apply Lemma \ref{lemma:3} to fuse the whole GPA procedure into one operator.

% \subsubsection{Backward Fusion}
% There is only one intermediate variable needed for backward propagation in the GPA procedure: $\boldsymbol{M}$, which can be recomputed within $O(1)$, so the recompute technique is applied.

% \subsubsection{Evaluation}
% Before fusion, there are 3 neural operators and 2 graph operators. The total memory space for saving the intermediate variable is $2f^{(l+1)}n+\left(f^{(l)}+2f^{(l+1)}\right)e$.

% After reorganization and fusion, there are 2 neural operators and 1 graph operators. The total memory space occupied is reduced to $3f^{(l+1)}n$.




==> tex/method-fusion.tex <==
\section{Reducing IO with Fusion under Unified Thread Mapping Scheme}
\subsection{Decoupling Thread Mapping Scheme from Operator}

\subsubsection{Operator: Node-centric and Edge-centric}
\textbf{Node-centric (NC)}: ApplyVertex,Gather.

\textbf{Edge-centric (EC)}: ApplyEdge,Scatter


\subsubsection{Scheme: Node-balance and Edge-balance}
 We use the concept of worker to represent parallel processing units(e.g., threads or warps) in this section. For GNN operators, there are generally two ways to assign the workload to workers: 

\textbf{Node-balance (NB)}: Assign a certain number of nodes to process in one worker, e.g., all edge values that share the same source or destination. 
% Compared with EB, NB method has no extra computation cost, but will result in an imbalanced workload between workers when the number of edges among nodes is imbalanced.

\textbf{Edge-balance (EB)}. Assign a certain number of edges to process in one worker, which will provide fine-grained parallelism and balanced workloads among workers. 
% However, EB method will introduce some extra cost under certain conditions. For instance, in SPMM, 
extra cost includes calculating the index for non-zero elements and atomic sum among workers.

\subsubsection{Combining Operator and Scheme}
There are four combinations for operators and schemes: NB scheme for NC operator, EB scheme for EC operator, NB scheme for EB operator, and EB scheme for NB operator.

NB for NC and EB for EC. These are the most natural and trivial situation

NB for EC. We allocate the 

\subsection{Unified Thread Mapping for Operator Fusion}

\subsection{Example with GATConv}





% In Section \ref{subsec:op abstract}, we defined meta operator type by the mapping relationship between input and output, and illustrate how to implement the operator with NB or EB method. Based on our meta operator abstraction, we formulate a set of rules for operator fusion and we will illustrate how to fuse the \textit{Scatter-ApplyEdge-Aggregate} procedure into one fused operator by our operator fusion rules.

% Our main idea is that given two operators with their meta operator type, we can find a way to: 1) determine the meta operator type of the fused operator; and 2) implement the fused operator with EB or NB method. Moreover, we perform the fusion technique over and over again until the whole \textit{Scatter-ApplyEdge-Aggregate} procedure is fused into one operator. The operator fusion rules are summarized in Table \ref{tab:fusion rules}.

% \begin{table*}
%     \centering
%     \scalebox{0.75}{
%     \begin{tabular}{|c|c|c|c|c|c|c|}
%         \hline
%          \diagbox{first op}{second op} & one-edge-to-edge & many-edge-to-edge & node-to-edge & edge-to-node & one-node-to-node & many-node-to-node \\
%          \hline
%          one-edge-to-edge & one-edge-to-edge & many-edge-to-edge & X & edge-to-node & X & X \\
%          \hline
%          many-edge-to-edge & many-edge-to-edge & many-edge-to-edge & X & edge-to-node & X & X\\
%          \hline
%          node-to-edge & node-to-edge & node-to-edge & X & many-node-to-node & X & X\\
%          \hline
%          edge-to-node & X & X & X & X & not profitable & X\\
%          \hline
%          one-node-to-node & X & X & not profitable & X & one-node-to-node & not profitable\\
%          \hline
%          many-node-to-node & X & X & X & X & not profitable & X\\
%          \hline

%     \end{tabular}}
%     \caption{Operator fusion rules. The first column and first row show the data mapping type of the first and second operators before fusion, and the cells show the data mapping type of the operator after fusion.}
%     \label{tab:fusion rules}
% \end{table*}

% We take some representatives from Table \ref{tab:fusion rules} and illustrate how to fuse these operators as the Table shows. Here we define $Op_1$ and $Op_2$ as the first and second operator, and $f_1$ and $f_2$ as their mapping function respectively.

% \textbf{Node-to-Edge with One-Edge-to-Edge.} One edge is mapped to one thread. In $Op_1$, each thread selects the node feature according to the graph structure and generate an edge feature with $f_1$ as output. In $Op_2$, each thread reads an edge feature and transform it into a new edge feature with $f_2$ as output. When a Node-to-Edge operator is fused with a One-Edge-to-Edge operator, each thread selects the node feature, then perform $f_1$ and $f_2$ sequentially to generate the output, which is overall a node-to-edge operator. By perform operator fusion, one write and one read to the DRAM are saved for each edge.

% \textbf{One-Edge-to-Edge with Many-Edge-to-Edge.} In $Op_1$, we map one thread to one edge, and each thread performs $f_1$ to an edge feature. In $Op_2$, one block is mapped to one neighborhood , one thread is mapped to an edge. When a One-Edge-to-Edge operator is fused with a Many-Edge-to-Edge, each thread first performs $f_1$, then all the threads in the block perform $f_2$. If we take $f_1$ as a part of $f_2$, the fused operator is Many-Edge-to-Edge, and one write and one read to the DRAM are saved for each edge.

% \textbf{Many-Edge-to-Edge with Edge-to-Node.} In $Op_1$, we assign one block for one neighborhood and one thread for every edge in the neighborhood. In $Op_2$, we assign one block to update one node feature and one thread to update one element in the feature vector. Each thread first perform $f_1$ and write the edge value to shared memory. After a block-level synchronization, each thread read from the shared memory and update its corresponding element. The fused operator is Edge-to-Node, and one write and one read to the DRAM are saved for each edge.


% \subsection{Examples}
% \subsubsection{GATConv}\label{gatconv:fuse}
% We perform operator fusion on the basis of operator reorganization in Section \ref{gatconv:reorg}. According to Table \ref{tab:fusion rules}, there are four operators that have a potential to fuse: 
% \begin{itemize}
%     \item a Node-to-Edge operator $\operatorname{u\_add\_v}$
%     \item a One-Edge-to-Edge operator $\operatorname{LeakyReLU}$
%     \item a Many-Edge-to-Edge operator $\operatorname{edge\_softmax}$
%     \item an Edge-to-Node operator $\operatorname{reduce\_sum}$
% \end{itemize}

% We fuse these four operators into one Many-Node-to-Node operator as follows. We assign one block to update each node, and one thread for each edge belonging to the neighborhood of this node. Each thread first read the feature of the source node and destination node of its edge and compute $\operatorname{u\_add\_v}$, then perform  $\operatorname{LeakyReLU}$. After that, a reduction is performed to compute the exponential sum in $\operatorname{edge\_softmax}$, and the final edge value is stored in shared memory. A $\operatorname{spmm-like}$ kernel is then performed with the edge values in shared memory to compute $\operatorname{reduce\_sum}$.

% The fused operator is overall Many-Node-to-Node, where each block take all the nodes in the neighborhood of one node as input and update this node as output. By operator fusion, we save three $O(|\mathcal{E}|)$ write and read to DRAM for each GATConv layer.

% \subsubsection{EdgeConv}
% We perform operator fusion on the basis of operator reorganization in Section \ref{edgeconv:reorg}. According to Table \ref{tab:fusion rules}, there are two operators that have a potential to fuse:
% \begin{itemize}
%     \item a Node-to-Edge operator $\operatorname{u\_add\_v}$
%     \item a Edge-to-Node operator $\operatorname{reduce\_max}$
% \end{itemize}

% We can fuse these two operators into one Many-Node-to-Node operator similar to Section \ref{gatconv:fuse}. One block is assigned to update each node and each thread in the block is responsible for one edge. Each thread first read the source node and destination node to compute $\operatorname{u\_add\_v}$ and store the result in shared memory. A $\operatorname{spmm-like}$ kernel is then performed to compute $\operatorname{reduce\_max}$. Compared with the non-fused implementation, $O(|\mathcal{E}|)$ write and read to DRAM are saved for each EdgeConv layer.


% \subsubsection{GMMConv}

% \begin{theorem}
%     The Generation-Passing-Aggregation procedure can be fused into one operator.
% \end{theorem}
    
% \begin{proof}
% The message-generation phase is one node-to-edge meta operator. Operators in message-passing phase are a sequence of one-edge-to-one-edge and many-edge-to-many-edge meta operators , which can be fused into one edge-to-edge meta operator by Lemma \ref{lemma:4}, \ref{lemma:5} and \ref{lemma:6}. Then the Generation phase and Passing phase can be fused into one node-to-edge operator by Lemma \ref{lemma:1} and \ref{lemma:2}. The Aggregation phase is one edge-to-node meta operator. By Lemma \ref{lemma:3}, the Aggregation phase can be fused with the fused Generation and Passing phase and all the GPA procudure is fused into one node-to-node operator.
% \end{proof}


